A Normal Distribution Transform-Based Radar Odometry Designed For Scanning and Automotive Radars

Existing radar sensors can be classified into automotive and scanning radars. While most radar odometry (RO) methods are only designed for a specific type of radar, our RO method adapts to both scanning and automotive radars. Our RO is simple yet effective, where the pipeline consists of thresholding, probabilistic submap building, and an NDT-based radar scan matching. The proposed RO has been tested on two public radar datasets: the Oxford Radar RobotCar dataset and the nuScenes dataset, which provide scanning and automotive radar data respectively. The results show that our approach surpasses state-of-the-art RO using either automotive or scanning radar by reducing translational error by 51% and 30%, respectively, and rotational error by 17% and 29%, respectively. Besides, we show that our RO achieves centimeter-level accuracy as lidar odometry, and automotive and scanning RO have similar accuracy.

==> Algorithm1.tex <==
\scalebox{0.9}{
\begin{algorithm}[H]
 \caption{Matching \label{algorithm:1}}
 %\begin{algorithmic}[1]
\textbf{Input:} Two radar scans $S_1, S_2$; default grid size $g_{init}$; and threshold value $thres$\\
\textbf{Output:} Transformation between two radar scans $T$

\SetAlgoLined

 \eIf{velocity$ < 1.5 km/hr$}{
   \STATE $g\gets 1.5m$\;}
   {
   \STATE $g\gets g_{init}$\;}
 
 \STATE $shift\gets thres$\;
 \STATE $T\gets$ DoNDTMatching($S_1$, $S_2$, $g$, $shift$)\;

 \While{$T$ does not match with motion prior}{
  \STATE $g\gets g+2.5m$\;
  \If{$g>12.5m$}{
   \STATE $g\gets g_{init}$\;
   \STATE $shift\gets shift/2$\;
   }
 
   \STATE $T\gets$ DoNDTMatching($S_1$, $S_2$, $g$, $shift$)\;
}
 %\end{algorithmic}
\end{algorithm}
}

==> tables/4Hz_vs._20Hz_LO.tex <==
\setlength{\arrayrulewidth}{0.2mm}
\setlength{\tabcolsep}{3pt}
%\setlength{\tabrowsep}{3pt}
\renewcommand{\arraystretch}{1.8}

\begin{table}[t]
\begin{center}
\scalebox{0.85}{

\begin{tabular}{ccccccccc}
\hline
               &  & \multicolumn{3}{c}{Frame-by-Frame Error} &  & \multicolumn{3}{c}{Per meter Error} \\ \cline{3-5} \cline{7-9} 
               &  & Translation     &      & Rotation        &  & Translation     &     & Rotation    \\
               &  & (m/frame)       &      & (deg/frame)     &  & (\%)            &     & (deg/m)     \\ \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
4Hz Lidar ICP  &  & 0.0617          &      & 0.0448          &  & 0.0814          &     & 0.0466      \\
20Hz Lidar ICP &  & 0.047           &      & 0.0357          &  & 0.1079          &     & 0.0687      \\ \hline
\end{tabular}

}
\end{center}
\caption{\label{tab:4Hz vs. 20Hz LO} Frame-by-Frame Error vs. Per meter Error.}
\end{table}

==> tables/RO_vs._LO.tex <==

\setlength{\arrayrulewidth}{0.2mm}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.5}

\begin{table}[t]
\begin{center}
\scalebox{0.85}{

\begin{tabular}{llclccccccc}
\hline
\multicolumn{1}{c}{Dataset}                 &  & Benchmarks           &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Translation error\\ (m/frame)\end{tabular}} &                      & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Rotation error\\ (deg/frame)\end{tabular}} \\ \cline{1-1} \cline{3-3} \cline{5-7} \cline{9-11} 
                                            &  &                      &  & Mean                         &                              & Std.                        &                      & Mean                         &                             & Std.                        \\ \cline{5-5} \cline{7-7} \cline{9-9} \cline{11-11} 
\multicolumn{1}{c}{\multirow{2}{*}{Oxford}} &  & Lidar ICP            &  & \textbf{0.0617}              &                              & 0.0620                      &                      & \textbf{0.0448}              &                             & 0.0652                      \\
\multicolumn{1}{c}{}                        %&  & Lidar NDT            &  & 0.0643                       &                              & 0.0640                      &                      & 0.0504                       &                             & 0.0698                      \\
\multicolumn{1}{c}{}                        &  & Scanning RO          &  & 0.0652                       &                              & 0.0581                      &                      & 0.0736                       &                             & 0.1106                      \\
                                            &  & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}        \\
\multirow{2}{*}{nuScenes}                   &  & Lidar ICP            &  & \textbf{0.0240}              &                              & 0.0198                      &                      & \textbf{0.0488}              &                             & 0.0429                      \\
                                            %&  & Lidar NDT            &  & 0.0401                       &                              & 0.1182                      &                      & 0.0676                       &                             & 0.0603                      \\
                                            &  & Automotive RO        &  & 0.0355                       &                              & 0.0227                      &                      & 0.1043                       &                             & 0.1429                      \\ \hline
\end{tabular}

}
\end{center}
\scriptsize
%\tiny
 \\
To have an equitable comparison with radar, we only calculate the SE2 error of Lidar odometry. 
%For the nuScenes dataset, we downsample 13Hz automotive radar and 20Hz Lidar to 4.33Hz and use ego-pose provided by nuScenes as ground truth. For the Oxford dataset, we downsample 20Hz Lidar to 4Hz and use GPS/INS provided by the Oxford dataset as ground truth. 
To get a good Lidar odometry performance, we employ fine-tuned multi-stage ICP and remove Lidar points on the ego-vehicle and Lidar rings on the ground by setting a fixed spatial threshold.
\caption{\label{tab:RO vs. LO} Radar Odometry vs. Lidar Odometry.}
\end{table}





==> tables/RO_vs._LO_new.tex <==
\setlength{\arrayrulewidth}{0.2mm}
\setlength{\tabcolsep}{2.3pt}
\renewcommand{\arraystretch}{1.6}

\begin{table}[t]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{clccccccc}
\hline
                              &  & \multicolumn{3}{c}{nuScenes Dataset} &  & \multicolumn{3}{c}{Oxford Dataset} \\ \cline{3-5} \cline{7-9} 
\multicolumn{1}{l}{} &  & \multicolumn{3}{c}{Automotive Radar} & \multicolumn{1}{l}{} & \multicolumn{3}{c}{Scanning Radar} \\ \cline{3-5} \cline{7-9} 
\multirow{2}{*}{Benchmarks}   &  & Trans.        &     & Rot.           &  & Tran.        &     & Rot.          \\
                              &  & (m/frame)     &     & (deg/frame)    &  & (m/frame)    &     & (deg/frame)   \\ \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
Lidar odometry                        &  & \textbf{0.0240}        &     & \textbf{0.0488}         &  & \textbf{0.0617}       &     & \textbf{0.0448}        \\
Radar odometry                  &  & 0.0355        &     & 0.1043         &  & 0.0652       &     & 0.0736        \\ \hline% \cline{1-1} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
%Error raised from LO to RO (\downarrow) &  & 47.92\%       &     & 113.73\%       &  & 5.67\%       &     & 64.27\%       \\ \hline
\end{tabular}
}
\end{center}
\scriptsize
%To compare the odometry performance between radar and lidar, we downsample all sensors to approximate 4Hz, evaluate the odometry performance by the frame-by-frame error, and only calculate the SE2 error of Lidar odometry.
%For the nuScenes dataset, we downsample 13Hz automotive radar and 20Hz Lidar to 4.33Hz and use ego-pose provided by nuScenes as ground truth. For the Oxford dataset, we downsample 20Hz Lidar to 4Hz and use GPS/INS provided by the Oxford dataset as ground truth. 
The lidar odometry is achieved by the fine-tuned multi-stage ICP. The lidar points on the ego-vehicle and ground are removed by a fixed spatial threshold. 
To have an equitable comparison with radar, we only calculate the SE2 error of lidar odometry.

\caption{\label{tab:RO vs. LO} Radar Odometry vs. Lidar Odometry.}
\vspace{-2.5mm}
\end{table}
